Expanded calculations of pn-QRPA electron capture rates on $^{55}$Co for presupernova and supernova physics

Due to its abundance and its relatively high capture rates, $^{55}$Co is one of the key nuclide that can control the dynamics of core collapse of a massive star. Previously we introduced our microscopic calculations of capture rates on $^{55}$Co using the proton-neutron quasi-particle random phase approximation (pn-QRPA) theory. Here we present for the first time an expanded calculation of the electron capture rates on $^{55}$Co on an extensive temperature-density scale. These type of scale is appropriate for interpolation purposes and of greater utility for simulation codes.

==> Captions.tex <==
\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\textwidth]{fig1}
\end{tabular}
\end{center}
\caption{Electron capture rates on $^{55}$Co, as function of
temperature for different selected densities . Densities are in
units of $g-cm^{-3}$. Temperatures are measured in $10^{9}$ K and
$log\lambda_{ec}$ represents the log of electron capture rates in
units of $Sec^{-1}$.

}\label{figure1}
\end{figure}
\newpage


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\textwidth]{fig2}
\end{tabular}
\end{center}
\caption{Cumulative sum of the B(GT+) values in $^{55}$Co. The
quenching factor $(0.74)^{2}$is included in the
calculations.}\label{figure2}
\end{figure}

\end{document}
\bye 

